Evolution of Digital Advertising Strategies during the 2020 US Presidential Primary

Political advertising on digital platforms has grown dramatically in recent years as campaigns embrace new ways of targeting supporters and potential voters. Previous scholarship shows that digital advertising has both positive effects on democratic politics through increased voter knowledge and participation, and negative effects through user manipulation, opinion echo-chambers, and diminished privacy. However, research on election campaign strategies has focused primarily on traditional media, such as television. Here, we examine how political campaign dynamics have evolved in response to the growth of digital media by analyzing the advertising strategies of US presidential election campaigns during the 2020 primary cycle. To identify geographic and temporal trends, we employ regression analyses of campaign spending across nearly 600,000 advertisements published on Facebook. We show that campaigns heavily target voters in candidates' home states during the "invisible primary" stage before shifting to states with early primaries.

==> tableex2.tex <==
\begin{table*}[htp!] \centering \footnotesize
  \caption{Panel Linear Model of the Full Sample of Data to Show Long Tables} 
  \label{tab:plmdata} 
\begin{tabular}{@{\extracolsep{5pt}}lcccc} 

 & \multicolumn{4}{c}{\textsl{Dependent variable: $log(Dependent Variable_{t-1} + 1)$}} \\ 
\cline{2-5} 
\\[-1.8ex] & (1) & (2) & (3) & (4) \\ 
\hline \\[-1.8ex] 
  Variable q  & $-$0.512 & $-$0.674 & $-$0.421 & $-$0.374 \\ 
  & (0.510) & (0.525) & (0.517) & (0.537) \\ 
  Variable 2 & 1.108$^{***}$ & 0.798$^{***}$ & 0.784$^{***}$ & 0.703$^{**}$ \\ 
  & (0.288) & (0.283) & (0.275) & (0.288) \\ 
  Variable 3  & 0.200 & 0.202 & 0.304$^{**}$ & 0.285$^{**}$ \\ 
  & (0.138) & (0.139) & (0.139) & (0.138) \\ 
  Variable 4 &  & $-$0.766$^{***}$ & $-$1.036$^{***}$ & $-$0.982$^{***}$ \\ 
  &  & (0.254) & (0.255) & (0.251) \\ 
  Variable 5 &  & 0.120 & 0.232$^{*}$ & 0.260$^{*}$ \\ 
  &  & (0.127) & (0.134) & (0.138) \\ 
  Variable 6 &  & 0.341$^{***}$ & 0.395$^{***}$ & 0.357$^{***}$ \\ 
  &  & (0.071) & (0.072) & (0.072) \\  
  Variable 7 &  &  & 0.232$^{***}$ & 0.189$^{***}$ \\ 
  &  &  & (0.034) & (0.036) \\ 
  Variable 8 &  &  & 0.253$^{***}$ & 0.206$^{***}$ \\ 
  &  &  & (0.037) & (0.042) \\ 
  Variable 9 &  &  & 0.060$^{***}$ & 0.051$^{***}$ \\ 
  &  &  & (0.008) & (0.009) \\ 
  Variable 10 &  &  & $-$0.018$^{***}$ & $-$0.012$^{*}$ \\ 
  &  &  & (0.007) & (0.007) \\ 
  Variable 11 &  &  &  & 0.329$^{***}$ \\ 
  &  &  &  & (0.125) \\ 
  Variable 12 &  &  &  & $-$0.320$^{***}$ \\ 
  &  &  &  & (0.062) \\ 
  Variable 13 &  &  &  & $-$0.124$^{***}$ \\ 
  &  &  &  & (0.031) \\ 
  Variable 14 &  &  &  & $-$0.060 \\ 
  &  &  &  & (0.057) \\ 
  Variable 15 &  &  &  & $-$0.340$^{***}$ \\ 
  &  &  &  & (0.055) \\ 
  Variable 16 &  &  &  & $-$0.123$^{***}$ \\ 
  &  &  &  & (0.033) \\ 
  Variable 17 & 0.0002 & 0.001 & $-$0.001 & $-$0.0003 \\ 
  & (0.001) & (0.001) & (0.001) & (0.001) \\
  Variable 18 & 0.006$^{***}$ & 0.005$^{***}$ & 0.012$^{***}$ & 0.011$^{***}$ \\ 
  & (0.001) & (0.001) & (0.001) & (0.001) \\ 
  Variable 19 & $-$0.129$^{***}$ & $-$0.123$^{***}$ & $-$0.039 & $-$0.036 \\ 
  & (0.032) & (0.032) & (0.034) & (0.036) \\ 
  Variable 20 & 0.629$^{***}$ & 0.624$^{***}$ & 0.598$^{***}$ & 0.618$^{***}$ \\ 
  & (0.010) & (0.010) & (0.010) & (0.011) \\ 
  Constant & 0.275$^{***}$ & 0.946$^{***}$ & $-$2.334$^{***}$ & $-$1.017$^{**}$ \\ 
  & (0.056) & (0.298) & (0.439) & (0.475) \\ 

\hline \\[-1.8ex] 
Obs. & 32,658 & 32,658 & 32,658 & 28,200 \\ 
Adj. R$^{2}$ & 0.371 & 0.374 & 0.389 & 0.429 \\ 
F Stat. & 2,756.800$^{***}$  & 1,949.369$^{***}$  & 1,485.940$^{***}$  & 1,058.683$^{***}$  \\ 
\hline \\[-1.8ex] 
\textsl{Note:}  & \multicolumn{4}{l}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table*}  
